The gradient flow running coupling with twisted boundary conditions

We study the gradient flow for Yang-Mills theories with twisted boundary conditions. The perturbative behavior of the energy density $\langle E(t)\rangle$ is used to define a running coupling at a scale given by the linear size of the finite volume box. We compute the non-perturbative running of the pure gauge $SU(2)$ coupling constant and conclude that the technique is well suited for further applications due to the relatively mild cutoff effects of the step scaling function and the high numerical precision that can be achieved in lattice simulations. We also comment on the inclusion of matter fields.

==> int.tex <==
We
checked that different integrators have the expected scaling by first
performing a very precise integration of an $L/a=8$ configuration
($\beta=2.8$) to a flow time $t=1$. This configuration at $t=1$ (let's
call it $V_\mu(x,t=1)$) is
compared with the result of different integration schemes and
different step sizes. If $V_\mu'(x,t=1)$ is the integrated
configuration with some scheme and step size, the error made by
integrating the flow equations is quantified by
\begin{equation}
  d = \max_{x,\mu}\left\{ {\rm dist}(V_\mu(x,t),
    V_\mu'(x,t)) \right\}   \,,
\end{equation}
where the distance between two $N\times N$ matrices $A_{ij}$ and
$B_{ij}$ is defined as 
\begin{equation}
  {\rm dist}(A,B) = \frac{1}{N^2}\sqrt{\sum_{i,j}|A_{ij} - B_{ij}|^2} \,.
\end{equation}

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{fig/error}
  \caption{Error made by different integration schemes as a function
    of the integration step size (in $\log-\log$ scale). The slopes of
  the linear fits are 1.0015(3) (Euler), 2.0025(9)
  (RK2), 2.031(8) (Heun), 3.04(1) (RK3).}
  \label{fig:int}
\end{figure}

Figure~\ref{fig:int} shows that the different schemes have the expected
scaling with the integration step size.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

